RENOVI: A Benchmark Towards Remediating Norm Violations in Socio-Cultural Conversations

Norm violations occur when individuals fail to conform to culturally accepted behaviors, which may lead to potential conflicts. Remediating norm violations requires social awareness and cultural sensitivity of the nuances at play. To equip interactive AI systems with a remediation ability, we offer ReNoVi - a large-scale corpus of 9,258 multi-turn dialogues annotated with social norms, as well as define a sequence of tasks to help understand and remediate norm violations step by step. ReNoVi consists of two parts: 512 human-authored dialogues (real data), and 8,746 synthetic conversations generated by ChatGPT through prompt learning. While collecting sufficient human-authored data is costly, synthetic conversations provide suitable amounts of data to help mitigate the scarcity of training data, as well as the chance to assess the alignment between LLMs and humans in the awareness of social norms. We thus harness the power of ChatGPT to generate synthetic training data for our task. To ensure the quality of both human-authored and synthetic data, we follow a quality control protocol during data collection. Our experimental results demonstrate the importance of remediating norm violations in socio-cultural conversations, as well as the improvement in performance obtained from synthetic data.

==> 1-intro.tex <==
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Outline:
% Para 1: Background of Socio-cultural Conversations, why important?

% Para 2: social norms can vary by culture, thereby norm violations can arise accidentaly. Remediatie norm violations in socia-cultural conversations is challenging. 

% Para 3: To bridge the research gap, we propose a dataset.

The rapid advance of globalization  has facilitated faster and more accessible communication among individuals who have different social or cultural backgrounds~\cite{castells2000toward,steger2017globalization}.
Social norms are pre-defined culturally acceptable boundaries for human behaviors that vary across cultures~\cite{fung2022normsage,ziems2023normbank,moghimifar2023normmark}.
Failing to adhere to such culturally accepted behaviors can lead to \textit{norm violations}, which negatively impact social interactions, \eg\ leading to misunderstandings and potential conflicts~\cite{triandis1994culture,hovy2021importance}.
As dialogue agents' participation in people's lives increases, they will increasingly operate within cultural and social spaces. Therefore, it
is essential to endow dialogue systems with the ability to detect and remediate norm violations.

%Understanding the impact of social norms is imperative on socio-cultural conversations. Social norms are pre-defined culturally acceptable boundaries for human behaviors~\cite{} that vary differently across cultures. Therefore, violations of social norms can arise frequently due to social or cultural differences. Whereas, failing to adhere to social norms can negatively impact social interactions~\cite{}, resulting in misunderstandings, conflicts, and potential harm to social relationships. 

Current work exploring social norms in conversations include norm discovery~\cite{fung2022normsage}, 
normative reasoning~\cite{forbes2020social} and moral and ethics judgements~\cite{ziems2022moral}.
However, these works mainly focus on extracting norms from context-response pairs, and cannot handle 
multi-turn conversations where adherence to social norms is important. 
\trackIZ{\citet{zhan2023socialdial} present a multi-turn dialogue corpus that includes social factors
(\eg \textit{social distance} and \textit{formality}) and users' behaviours (\eg \textit{greeting}
and \textit{critism}), which is used to detect norm violations.}\noteIZ{I rewrote this. Plz check} 
However, none of these works shed light on how to remediate norm violations in conversations.

\input{emnlp2023-latex/figures/intro-framework}

To bridge this research gap, we introduce the \ourframework\ framework to explore how to 
remediate norm violations in cross-cultural conversations, where adherence to social norms is important. 
As shown in Figure~\ref{fig:intro}, the \ourframework\ framework decomposes the analysis 
of norm violations into four sub-tasks: (1)~norm violation detection, (2)~impact estimation, 
(3)~remediation generation, and (4)~justification generation. To facilitate the research 
on this task, we construct a large-scale socio-cultural dialogue corpus \ourdata.
In our work, \ourdata\ focuses on the social norms in Chinese culture.
%%, a country with a history spanning 5,000 years. 
\ourdata\ contains 9,512 multi-turn dialogues in total, including 512 human-authored 
dialogues and 9.5K synthetic dialogues generated by ChatGPT. The human-authored corpus provides
fine-grained annotations covering norm category, violation status, impact of violation, 
remediation and justification. However, we need additional data to train our models, and 
collecting suitable amounts of data by crowd-sourcing is both time consuming and expensive. 
\trackIZ{Since, synthetic data generated by ChatGPT has been shown to be an effective way to relief data scarcity,}\noteIZ{citations} 
we devise an ontology-based method to prompt ChatGPT in order to generate synthetic training data.
To ensure the quality of both human-authored and synthetic data, \trackIZ{we have performed extensive 
quality control during data collection.}\noteIZ{if this is described in the paper, refer to the section; if not, remove the sentence}

The quality of the ChatGPT-generated dialogues is evaluated through experiments on \trackIZ{four
sub-tasks.}\noteIZ{Which ones?} 

Our main contributions are:
\begin{itemize}
    \item We propose a \textsc{Normvr} framework and corresponding \ourdata dataset to explore how to remediate norm violations in \trackIZ{socio-cultural conversations,}\noteIZ{Huh?} \trackIZ{encompassing four aspects: norm violation detection, impact violation, remediation generation and justification generation.}\noteIZ{not clear who is incompassing these aspects}
    \item We conduct experiments to validate the effectiveness of our dataset, and verify that synthetic data can improve  performance in both four sub-tasks.
\end{itemize}

% \begin{itemize}
%     \item Impact estimation
%     \item Generation of remediation measures.
%     \item Generation of justifying remediation measures.
%     \item Ranking of remediation candidates.
%     \item Ranking of justification candidates.
% \end{itemize}

==> tables/norm_violation_class.tex <==


\begin{table}[!t]
\centering
\tiny
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{cc|lccc}
\hline
%\multicolumn{4}{c}{Training on human-annotated data}             \\ \hline
 Human &  Synthetic  & \textbf{Models}    & 
 \textbf{P}   & \textbf{R}   & \textbf{F1}   \\ \hline
 \checkmark &  & BERT-zh             & 59.68        & 58.92        & 59.30         \\
 \checkmark &  & RoBERTa-zh         & 66.86        & 65.70        & 66.27       \\ \hline
%%\multicolumn{4}{c}{Training on synthetic data}                   \\ \hline
  Human&  Synthetic  & \textbf{Models}    & 
 \textbf{P}   & \textbf{R}   & \textbf{F1}   \\ \hline
 &  \checkmark & BERT-zh            & 59.33        & 58.25        & 58.78       \\
 &  \checkmark & RoBERTa-zh          & 65.60        & 65.59        & 65.59     \\ \hline
%\multicolumn{4}{c}{Training on human-annotated + synthetic data} \\ \hline
  Human &  Synthetic  & \textbf{Models}    & 
 \textbf{P}   & \textbf{R}   & \textbf{F1}   \\ \hline
 \checkmark & \checkmark  & BERT-zh             & 71.04        & 68.34        & \textbf{69.66}       \\
 \checkmark &  \checkmark & RoBERTa-zh          & 67.99        & {66.97}        & \textbf{67.47}     \\ \hline
\end{tabular}%
%}
\caption{Experiment results of norm violation detection models trained on three different training settings.}
\label{tab:norm_violation_detection_results}
\end{table}

==> tables/reranking.tex <==
\begin{table}[!t]
    \centering
    \tiny
    \begin{tabular}{lcc}
    \toprule
      &\textbf{Remediation} & \textbf{Justification}  \\ 
             BERT-zh   & 12.34  & 23.14 \\
        BERT-zh +pfeiffer  &31.75 &  25.97    \\
       MiniLM-L12-v2   &  34.06 &  29.31 \\
        MiniLM-L12-v2 +pfeiffer  &31.55 &  27.52    \\
    \bottomrule
    \end{tabular}
    \caption{The accuracies of remediation and justification ranking, respectively.}
    \label{tab:rerank}
\end{table}
